SurgVLM: A Large Vision-Language Model and Systematic Evaluation Benchmark for Surgical Intelligence

Foundation models have achieved transformative success across biomedical domains by enabling holistic understanding of multimodal data. However, their application in surgery remains underexplored. Surgical intelligence presents unique challenges - requiring surgical visual perception, temporal analysis, and reasoning. Existing general-purpose vision-language models fail to address these needs due to insufficient domain-specific supervision and the lack of a large-scale high-quality surgical database. To bridge this gap, we propose SurgVLM, one of the first large vision-language foundation models for surgical intelligence, where this single universal model can tackle versatile surgical tasks. To enable this, we construct a large-scale multimodal surgical database, SurgVLM-DB, comprising over 1.81 million frames with 7.79 million conversations, spanning more than 16 surgical types and 18 anatomical structures. We unify and reorganize 23 public datasets across 10 surgical tasks, followed by standardizing labels and doing hierarchical vision-language alignment to facilitate comprehensive coverage of gradually finer-grained surgical tasks, from visual perception, temporal analysis, to high-level reasoning. Building upon this comprehensive dataset, we propose SurgVLM, which is built upon Qwen2.5-VL, and undergoes instruction tuning to 10+ surgical tasks. We further construct a surgical multimodal benchmark, SurgVLM-Bench, for method evaluation. SurgVLM-Bench consists of 6 popular and widely-used datasets in surgical domain, covering several crucial downstream tasks. Based on SurgVLM-Bench, we evaluate the performance of our SurgVLM (3 SurgVLM variants: SurgVLM-7B, SurgVLM-32B, and SurgVLM-72B), and conduct comprehensive comparisons with 14 mainstream commercial VLMs (e.g., GPT-4o, Gemini 2.0 Flash, Qwen2.5-Max).

==> Parts/methods.tex <==
\section{Method}
In this section, we describe the underlying architecture of our model and the techniques employed to enhance its capabilities for surgical AI applications.

\subsection{Base Model: Qwen2.5}
Our model is built upon Qwen2.5, a high-performance open-weight large language model (LLM) designed for multimodal reasoning. Qwen2.5 follows a decoder-only transformer architecture, a design widely adopted by models such as GPT-3 and Qwen's own series of LLMs due to its efficiency in handling sequential data and autoregressive generation.
Decoder-only architectures are particularly advantageous for multimodal applications, as they generate outputs autoregressively, making them well-suited for tasks that require structured reasoning and response generation. Unlike encoder-only models, which focus on representation learning, and encoder-decoder models, which introduce additional complexity for sequence transduction, the decoder-only framework allows for efficient multiturn interactions and seamless integration of vision and language inputs. This enables effective surgical QnA modeling, instruction tuning, and procedural reasoning.

\subsubsection{Model Adaptation}
Although Qwen2.5 has been pretrained on a large-scale corpus encompassing general-purpose and domain-specific data, direct application to the surgical domain remains challenging. Surgical reasoning requires precise domain knowledge, multimodal comprehension, and structured procedural reasoning, making general-purpose LLMs suboptimal.
To bridge this gap, we do not rely on end-to-end fine-tuning, which is often impractical due to the limited availability of annotated surgical datasets. Instead, we employ instruction tuning, an efficient adaptation strategy that enables the model to generalize across surgical tasks while requiring significantly fewer domain-specific training samples. By leveraging structured QnA-based supervision and multimodal alignment, we enhance the model's ability to interpret surgical workflows, reason over procedural steps, and generate clinically relevant responses.

\subsubsection{Projector Pretraining}
To ensure seamless vision-language integration, we introduce projector pretraining, aligning visual and textual modalities in the model's latent space. The vision encoder, based on SigLIP-400M, processes surgical images, while a projection layer maps visual representations to match textual embeddings. This enables effective cross-modal grounding, which is crucial for surgical applications.

The pretraining strategy consists of two phases. First, image captioning pretraining teaches the model to generate structured descriptions of surgical images, reinforcing associations between anatomical structures, surgical instruments, and procedural elements. Second, visual question answering (VQA) pretraining enhances structured multimodal reasoning, conditioning textual responses on surgical images to improve situational understanding.

By incorporating projector pretraining, we establish a unified multimodal representation, allowing the model to generate accurate surgical responses grounded in both vision and language.

\subsubsection{Instruction Tuning}
Following projector pretraining, we refine the model using instruction tuning, which aligns it with surgical reasoning, multimodal understanding, and structured procedural workflows. Unlike end-to-end fine-tuning, which requires large datasets, instruction tuning provides a scalable and efficient adaptation strategy.

A key enhancement in this phase is the semantic extension with surgical explanations, where textual descriptions of surgical types, tool interactions, and anatomical structures reinforce the model's ability to interpret complex workflows. Traditional image-text alignment often lacks sufficient domain specificity, making it ineffective for surgical AI tasks. To address this, we integrate stepwise surgical reasoning, which explicitly links textual outputs with visual inputs, allowing the model to learn structured associations between phases, instruments, and anatomical regions.

To ensure task generalization, instruction tuning includes multiple formats, such as multiple-choice QnA and sentence-based responses. This diversity prevents format-specific biases, enabling the model to handle classification tasks, workflow reasoning, and procedural descriptions. Furthermore, we incorporate multi-turn reasoning, where related surgical queries are merged to simulate real-world reasoning processes, ensuring the model can maintain contextual coherence across different procedural stages.

We also integrate hierarchical instruction tuning, structuring surgical questions to preserve task dependencies. Instead of treating individual queries as independent tasks, this technique enables progressive learning of procedural steps, ensuring logical consistency in the model's reasoning.

Finally, to improve cross-task generalization, we introduce mixture instruction learning, merging interrelated surgical instructions into a structured framework. This enables the model to handle instrument recognition, workflow reasoning, and surgical reasoning without requiring separate fine-tuning for each subtask. By enforcing response consistency across multiple instruction types, we ensure robust and reliable performance in multimodal surgical AI applications.

By integrating projector pretraining and instruction tuning, the final model achieves robust multimodal reasoning, structured surgical QnA comprehension, and efficient response generation, making it well-suited for surgical guidance, workflow analysis, and clinical decision support.
